Superconductivity beyond the Pauli limit in high-pressure CeSb2

We report the discovery of superconductivity at a pressure-induced magnetic quantum critical point in the Kondo-lattice system CeSb2, sustained up to magnetic fields that exceed the conventional Pauli limit eight-fold. Like CeRh2As2, CeSb2 is locally non-centrosymmetric around the Ce-site, but the evolution of critical fields and normal state properties as CeSb2 is tuned through the quantum critical point motivates a fundamentally different explanation for its resilience to applied field.

==> Significance.tex <==
% !TEX root = CeSb2V4.tex
% Superconductivity resilient to high magnetic fields is a key signature of unusual pairing states, because it indicates that the superelectrons form spin-triplet Cooper pairs. Such pairing states offer a handle for topological quantum computing, but they are difficult to resolve experimentally. New insights into this long-standing problem arise from our discovery and investigation of superconductivity in CeSb$_2$, which emerges near the threshold of magnetism at high pressure out of a highly anomalous normal state and reaches to fields that exceed the conventional Pauli limit by at least a factor of eight. 
% CeSb$_2$ is locally non-centrosymmetric around the Ce-site, a structural peculiarity that is thought to underpin the  field-resilience of several other unconventional superconductors, but
% the observed evolution of critical fields and normal state properties, as CeSb$_2$ is tuned through the threshold of magnetism under applied pressure and magnetic field, invites an alternative and more general explanation for its large upper critical field.

%Because CeSb$_2$ shares an important structural peculiarity with other field-resilient superconductors our findings offer a timely perspective on a wide family of unusual materials of current interest.
Superconductivity resilient to high magnetic fields signals spin-triplet pairing. Such unconventional pairing states offer attractive applications in topological quantum computing, but they are difficult to identify experimentally. New insights into this long-standing problem arise from our discovery of superconductivity in pressurised CeSb2, which  reaches to fields that far exceed the conventional Pauli limit. 
CeSb2 is locally non-centrosymmetric around the Ce-site. This property is thought to underpin the field-resilience of other systems such as CeRh2As2, but our findings suggest a fundamentally different and more general explanation in CeSb2, introducing an intriguing new aspect to the discussion of superconductivity at high fields.

